Fast Sparse Decision Tree Optimization via Reference Ensembles

Sparse decision tree optimization has been one of the most fundamental problems in AI since its inception and is a challenge at the core of interpretable machine learning. Sparse decision tree optimization is computationally hard, and despite steady effort since the 1960's, breakthroughs have only been made on the problem within the past few years, primarily on the problem of finding optimal sparse decision trees. However, current state-of-the-art algorithms often require impractical amounts of computation time and memory to find optimal or near-optimal trees for some real-world datasets, particularly those having several continuous-valued features. Given that the search spaces of these decision tree optimization problems are massive, can we practically hope to find a sparse decision tree that competes in accuracy with a black box machine learning model? We address this problem via smart guessing strategies that can be applied to any optimal branch-and-bound-based decision tree algorithm. We show that by using these guesses, we can reduce the run time by multiple orders of magnitude, while providing bounds on how far the resulting trees can deviate from the black box's accuracy and expressive power. Our approach enables guesses about how to bin continuous features, the size of the tree, and lower bounds on the error for the optimal decision tree. Our experiments show that in many cases we can rapidly construct sparse decision trees that match the accuracy of black box models. To summarize: when you are having trouble optimizing, just guess.

==> algsFromGosdt/extract.tex <==
\begin{algorithm}
\caption{extract$(t)$ $\rightarrow$ $s$ \comment{Extract optimal tree after running the algorithm}\label{alg:extraction}}
\begin{minipage}{1.0\linewidth}
\begin{tabbing}
xxx \= xxx \= xxx \= xxx \kill
\textbf{input:} $s$ \comment{Key of the problem from which we want to build a tree} \\
\textbf{output:} $t$ \comment{Optimal tree} \\
$p \leftarrow$ FIND\_OR\_CREATE\_NODE$(G,s)$ \comment{Find the node associated to this key} \\
$t \leftarrow$ None \comment{ Create a null tree } \\
$base\_bound \leftarrow p.ub$ \comment{ The risk if we end this node as a leaf } \\ 
$base\_prediction \leftarrow 0$ \comment{ The prediction if we end this node as a leaf } \\
$split\_bound \leftarrow \infty$ \comment{ The risk if we split this node } \\
$split\_feature \leftarrow 0$ \comment{ The index of the feature we should use to split this node } \\
\textbf{for} each feature $j \in [1,M]$ \textbf{do} \comment{ Check all possible features } \\
\> $s_l, s_r \leftarrow \text{split}(s,j,Z)$ \comment{Key of the the children for this split} \\
\> $p_l^j\leftarrow$FIND\_OR\_CREATE\_NODE$(G,s_l)$ \comment{Find left child} \\
\> $p_r^j\leftarrow$FIND\_OR\_CREATE\_NODE$(G,s_r)$ \comment{Find right child} \\
\> \comment{Check if the risk of this split is better than the best split risk so far } \\
\> \textbf{if} $p_l^j.ub + p_r^j.ub < split\_bound$ \textbf{then} \\
\> \> $split\_bound \leftarrow p_l^j.ub + p_r^j.ub$ \comment{ Update the best split risk } \\
\> \> $split\_feature \leftarrow j$ \comment{Best feature index to split on which minimizes loss upper bound} \\
\comment{ Calculate the total positive and negative weights of each equivalence class} \\
\textbf{for} each equivalence class $u \in [1,U]$ \textbf{define}\\
\> \comment{Values come from equivalence class matrix $Z$ as seen in Algorithm \ref{alg:upperbound}} \\
\> $z_u^- = \frac{1}{N}\sum_{i=1}^{N}\mathds{1}[y_i = 0 \land x_i = z_u]$ \comment {total negatives } \\
\> $z_u^+ = \frac{1}{N}\sum_{i=1}^{N}\mathds{1}[y_i = 1 \land x_i = z_u]$ \comment {total positives} \\
\comment{ Select only the positive and negative weights captured by $s$ } \\
$negatives \leftarrow \sum_u s_u z_u^-$ \\
$positives \leftarrow \sum_u s_u z_u^+$ \\
\comment{ Set the leaf prediction based on class with the higher selected total weight } \\
\textbf{if} $negatives < positives$ \textbf{then} \\
\> \comment{Leaf predicts the majority class as 1 since positive weights are higher} \\
\> $base\_prediction.pred \leftarrow 1$ \\
\comment{Base case: If the risk of remaining as a leaf is better than splitting, remain as leaf} \\
\textbf{if} $base\_bound \leq split\_feature$ \\
\> \comment{Construct and return a leaf node} \\
\> $t.type \leftarrow leaf$ \\
\> $t.prediction \leftarrow base\_prediction$ \\
\> \textbf{return} $t$ \\
\comment{Recursive case: One of the splits performs better than the leaf} \\
\comment{Generate left and right splits based on best split feature} \\
$s_l, s_r \leftarrow \text{split}(s,split\_feature,Z)$ \\
\comment{Recurse onto child keys to create left and right subtrees}\\
$t_l \leftarrow \text{extract}(s_l)$ \\
$t_r \leftarrow \text{extract}(s_r)$ \\
\comment{Construct and return a split node containing the left and right subtrees} \\
$t.type \leftarrow tree$ \\
$t.split \leftarrow split\_feature$ \\
$t.left \leftarrow t_l$ \\
$t.right \leftarrow t_r$ \\
\textbf{return} $t$
\end{tabbing}
\end{minipage}
\end{algorithm}

==> algsFromGosdt/fails_bounds.tex <==
\begin{algorithm}
\caption{fails\_bounds$(p)$ $\rightarrow$ $v$\label{alg:failsbound}}
\begin{minipage}{1.0\linewidth}
\begin{tabbing}
xxx \= xxx \= xxx \kill
\textbf{input:} $p$ \comment{current problem} \\
\textbf{output:} $v$ \comment{boolean indicating valid problem} \\
\comment{ If this expression is true then the lower bound on incremental accuracy is crossed by all descendents } \\
\comment{ This works because since $ub - lb$ is an upperbound on incremental accuracy for any descendent } \\
$incremental\_accuracy \leftarrow p.ub - p.lb \le \lambda$ \\
\comment{ If this expression is true then the lower bound on leaf classification accuracy is crossed } \\
$leaf\_accuracy \leftarrow p.ub \le 2\lambda$ \\
\textbf{if} $(incremental\_accuracy = True) \lor (leaf\_accuracy = True)$ \textbf{then} \\
\> \textbf{return} $True$ \\
\textbf{return} $False$\\
\end{tabbing}
\end{minipage}
\end{algorithm}

==> algsFromGosdt/split.tex <==
\begin{algorithm}
\caption{split$(s, j, Z)$ $\rightarrow$ $s_l, s_r$\label{alg:split}}
\begin{minipage}{1.0\linewidth}
\begin{tabbing}
xxx \= xxx \= xxx \kill
\textbf{input:} $s, j, Z$ \comment{support set, feature index, unique sample set} \\
\textbf{output:} $s_l, s_r$ \comment{left and right splits} \\
\comment{Create the left key which is the subset of $s$ such that feature $j$ tests negative} \\
$s_l = \{\mathds{1}[s_u = 1 \land Z_{u,j} = 0] | 1 \le u \le U\}$ \\
\comment{Create the right key which is the subset of $s$ such that feature $j$ tests positive} \\
$s_r = \{\mathds{1}[s_u = 1 \land Z_{u,j} = 1] | 1 \le u \le U\}$ \\
\textbf{return} $s_l, s_r$
\end{tabbing}
\end{minipage}
\end{algorithm}

==> algsFromGosdt/upper_bound.tex <==
\begin{algorithm}
\caption{get\_upper\_bound$(s, Z, z^-, z^+)$ $\rightarrow$ $ub$\label{alg:upperbound}}
\begin{minipage}{1.0\linewidth}
\begin{tabbing}
xxx \= xxx \= xxx \kill
\textbf{input:} $s, Z, z^-, z^+$ \comment{support, unique sample set, negative sample set, positive sample set} \\
\textbf{output:} $ub$ \comment{Risk upper bound} \\
\comment{Compute the risk contributed if applying a single class to all samples in $s$} \\
\textbf{for} each equivalence class $u \in [1,U]$ \textbf{define}\\
\> \comment{Add up the positive and negative class weights under equivalence class $u$} \\
\> $z_u^- = \frac{1}{N}\sum_{i=1}^{N}\mathds{1}[y_i = 0 \land x_i = z_u]$ \\
\> $z_u^+ = \frac{1}{N}\sum_{i=1}^{N}\mathds{1}[y_i = 1 \land x_i = z_u]$ \\
\comment{Total the positive and negatives over all classes $u$, choosing the smaller total as the misclassification} \\
\comment{Add a single $\lambda$ for the complexity penalty of a leaf} \\
$ub \leftarrow \lambda +\text{min}(\sum_u s_u z_u^-, \sum_u s_u z_u^+)$ \\
\textbf{return} $ub$
\end{tabbing}
\end{minipage}
\end{algorithm}

==> guessing_depth.tex <==
% Guessing Depth:
\def\x{\textbf{x}}
\def\y{\textbf{y}}

Many optimal decision tree algorithms optimize within a given depth constraint. Defining $f(t, d, \tilde{\x}, \y)$ as the objective function for some decision tree $t$, given binarized training data $\tilde{\x}$, training labels \y, and a user-provided depth constraint $d$, we have:
\[f(t, d, \tilde{\x}, \y) = \begin{cases} 
\mathcal{L} (t, \tilde{\x}, \y) & \text{depth}(t) \leq d \\
\infty & \text{depth}(t) > d
\end{cases}\]
%Where $\mathcal{L}(t, \tilde{\x}, \y)$ is some loss function for $t$ evaluated on the training set. A common choice for $\mathcal{L}$ is the misclassification error: the fraction of training data that are incorrectly classified by the tree $t$. 

%The depth constraint serves three key purposes. First, it keeps optimization feasible, by constraining the search space. Second, it makes optimization meaningful: the depth constraint keeps our decision trees simple enough to generalize, so that maximizing training accuracy translates to finding a model with high test accuracy. Third, it keeps our models interpretable, since trees that are too deep can be difficult to understand. All of these benefits, however, depend on a reasonable depth constraint. Allowing trees to be too deep removes all of the above benefits, but not allowing trees to be deep enough means that even the optimal solution might not be particularly accurate. When decision tree algorithms claim to be optimal, the functional meaning is that their solutions are likely to have high test accuracy, if they were optimized with a well-selected guess for the depth constraint.

Optimizing with depth constraints is powerful for several reasons: using a depth constraint not only makes it feasible to optimize with respect to training set error, it also makes optimization on a training set meaningful. Because a lower depth leads to a simpler model, the improvement in training set error that we get from optimizing is likely to match test error improvement, and the resulting models are likely to be human-interpretable. Users still have to be careful not to guess too low - then we just get a weak model - but this is a standard tradeoff that is present in all decision tree algorithms. When decision tree algorithms claim to be optimal, the functional meaning is that their solutions are likely to have high test accuracy, if they were optimized with a good guess for depth.
%be more diplomatic about saying "guess"? This may also go in the background

%Low depth constraints have benefits to generalizability, interpretability and run time. 


%Because depth alone does not fully describe the complexity of a decision tree, s
Optimizing with a hard depth constraint can lead to unduly complicated models, however. While a hard depth constraint is convenient for optimization, that loss does not differentiate between full trees whose depth matches the depth constraint and sparser, shallower trees with comparable accuracy. A hard depth constraint a) does not reward trees for being shallower than the maximum depth and b) only constrains trees by the length of their longest path, not any other measure of simplicity, like the length of the average path or the number of different decision paths. Ideally, a decision tree algorithm would output the simplest model that classifies the data well, since that leads to a more interpretable and generalizable model.
%we also sometimes need high depth models that aren't computationally feasible
%Yeah! depth alone can lead to unduly slow answers - right? depth constraint 10 is not something dl85 can do at all

%give a shorter version? Trust the background?
%One optimal decision tree algorithm, GOSDT, parameterizes simplicity by using a soft constraint on the number of leaves, instead of a hard constraint on depth.
One optimal decision tree algorithm, GOSDT, improves on model sparsity by optimizing with a soft constraint on the number of leaves instead of a hard depth constraint (see  Eq (\ref{eq:obj2})), but does so at the cost of run time. %Defining $g(t, \lambda, \tilde{\x}, \y)$ as the GOSDT-style objective function for some decision tree $t$, with number of leaves $H$ and non-negative regularization $\lambda$, we have: 
%\[g(t, \lambda, \tilde{\x}, \y) = \mathcal{L}(t,\tilde{\x},\y) + \lambda H \]
The key challenge with optimizing this loss is that the soft constraint from per-leaf regularization leads to a much larger search space than a hard depth-based constraint. GOSDT must consider deep, sparse trees alongside full, shallow ones. For example, if the regularization is set low enough to consider a full tree of depth 4 (16 leaves, if we take the root as depth 0) then the algorithm must also consider sparse trees up to depth 15, since there exists a depth 15 tree with only 16 leaves. \textcolor{red}{HM: Can we calculate/share the exact combinatorial complexity of a hard depth constraint vs a hard leaf constraint, or is that misleading since we have a soft constraint?} %todo: provide more detail for this example - the 1/16 -> 16 leaves rule? although idk, that seems a bit weird if a) we have >16 classes and can't do better than guessing at the root, so the default rule has objective, say, 16/17 + 1/16 > 1 or if b) we have 2 classes and know the loss is <= .5 + 1 leaf, so we can say something stronger
%we do penalize the root right?
%The algorithm can prune potential trees if the


%The issue with just using depth constraints as a guess is: doesn't capture full complexity, we gotta guess multiple constraints if we want to be confident we haven't made a bad guess, we gotta 
%sure we introduce more hyperparameters, but you can always just pick a couple to use if you don't want to cross-validate too many choices. It's no worse than not having them in the first place, and maybe researchers have intuition about which parameters are worth optimizing

%remove this paragraph, use in earlier pitch like the abstract?
%todo: use line below
%We can layer multiple constraints to better describe the space of trees that are simple enough to be interpretable and not overfit. 
%within which we should optimize. 

%fast, simple, accurate
By combining constraints on per-leaf sparsity and depth, we can make simple and accurate models quickly. To combine the constraints, we define a loss that is the maximum of the loss for depth budget algorithms and the loss for per-leaf regularized algorithms. That is%We define our new objective $R(t, \lambda, d, \tilde{\x}, \y)$, which is the maximum of $f$ and $g$ as defined above:
%Defining $R(d, x, y, b)$ as the regularized empirical risk for some decision tree d (with depth $D_d$ and number of leaves $H_d$)
\[R(t, \lambda, d, \tilde{\x}, \y) = \begin{cases} 
\mathcal{L}(t, \tilde{\x}, \y) + \lambda H & \text{depth}(t) \leq d \\
\infty & \text{depth}(t) > d
\end{cases}\]
For the right depth constraints, this simple adjustment yields orders of magnitude improvement in run time relative to GOSDT, and improves sparsity relative to DL8.5 %todo: update based on actual experiments

We think of this approach as using GOSDT's loss, but with a guess that at least one optimal tree for this loss is below depth $d$. If we are correct, we still find the optimal tree, and do so much more quickly than GOSDT would have. If we are incorrect, we still consider the same space of models as any depth-based decision tree algorithm. This approach does require a guess about depth to find the best tree, but so do all decision tree algorithms that use a hard constraint on depth. More importantly, it makes sense to make guesses in this context - they improve feasibility while encouraging the simplicity necessary for solutions to generalize. If we make a guess that is reasonable, but happens to be "wrong" - we prune the optimal tree as defined by our loss function - it could still be that the optimal tree was too complicated, and would have overfit. %see experiments

%post test error results, we can say something like faster, simpler, and better avoid overfitting while performing well on the training set. 
%make the intractable tractable?
%we can even turn one off altogether, or set it really loosely, and still get a reasonable answer
%
%do we discuss hyperparameter search? That's the big concern I have for this paper - we reduce the run time, sure, but we also introduce a greater range of guesses that someone would search over, so the full run time might still be a while (although at least we aren't in the "never finish" case as often)

==> lbguess/algorithm_guessing_lower_bound.tex <==
\definecolor{darkgreen}{rgb}{0.1, 0.6, 0.3}
\newcommand{\comment}[1]{\textcolor{darkgreen}{// #1}}
\begin{algorithm}
\caption{get\_lower\_bound$(s, Z, z^-, z^+)$ $\rightarrow$ $lb$\label{alg:lowerbound})}
\begin{minipage}{1.0\linewidth}
\begin{tabbing}
xxx \= xxx \= xxx \kill
\textbf{input:} $s, Z, z^-, z^+, \hat{y}^T$ \comment{support, unique sample set, negative sample set, positive sample set, reference predictions} \\
\textbf{output:} $lb$ \comment{Guessed risk lower bound} \\
\comment{Compute the risk if decision tree is guaranteed to make the same misclassifications as the black box} \\
$\textrm{guessed}\_lb \leftarrow \sum_{n \in s_a} \mathbf{1}[y_n \neq \hat{y}_n^{T}]$\\
\comment{Add a single $\lambda$ which is a lower bound of the complexity penalty} \\
$guessed\_lb \leftarrow \lambda + {guessed\_lb}$ \\
\comment{Compute the risk contributed if applying a class to every equivalance class independently (a guaranteed lower bound)} \\
\textbf{for} each equivalence class $u \in [1,U]$ \textbf{define}\\
\> \comment{Values provided in $Z$} \\
\> $z_u^- = \frac{1}{N}\sum_{i=1}^{N}\mathds{1}[y_i = 0 \land x_i = z_u]$ \\
\> $z_u^+ = \frac{1}{N}\sum_{i=1}^{N}\mathds{1}[y_i = 1 \land x_i = z_u]$ \\
\> \comment{Risk of assigning a class to equivalence class $u$} \\
\> $z_u^{\min} = \min(z_u^-, z_u^+)$ \\
\comment{Add all risks for each class $u$} \\
\comment{Add a single $\lambda$ which is a lower bound of the complexity penalty} \\
$guaranteed\_lb \leftarrow \lambda + \sum_u s_u z_u^{\min}$ \\
\comment{Handle case where guessed lower bound is below guaranteed} \\
$lb \leftarrow \max(guaranteed\_lb, guessed\_lb)$ \\
\textbf{return} $lb$
\end{tabbing}
\end{minipage}
\end{algorithm}
